Compactification de varietes de Siegel aux places de mauvaise reduction

We construct arithmetic toroidal compactifications of the moduli stack of principally polarized abelian varieties with parahoric level structure. To this end, we extend the methods of Faltings and Chai to a case of bad reduction. ----- Nous construisons des compactifications toroidales arithm\'etiques du champ de modules des vari\'et\'es ab\'eliennes principalement polaris\'ees munies d'une structure de niveau parahorique. Pour ce faire, nous \'etendons la m\'ethode de Faltings et Chai \`a un cas de mauvaise r\'eduction.

==> macros.tex <==
% macros pour LaTeX
% version du 2008-05-09
%personnalisé par Benoît

\newcommand{\courte}[3]{0\rightarrow #1 \rightarrow #2 \rightarrow #3 \rightarrow 0}
\newcommand{\Z}{\mathbb Z}
\newcommand{\Q}{\mathbb Q}
\newcommand{\R}{\mathbb R}
\newcommand{\C}{\mathbb C}
\newcommand{\F}{\mathbb F}
\newcommand{\A}{\mathbb A}
\newcommand{\Gm}{{\mathbb G}_m}

\newcommand{\Hom}{\underline{\mathrm{Hom}}}
\newcommand{\Ext}{\underline{\mathrm{Ext}}^1}

\newcommand{\OO}{\mathscr{O}} 		% faisceau structural

\newcommand{\Spec}{\mathrm{Spec}}

\newcommand{\iso}{\buildrel{\sim}\over\rightarrow}


%conflit avec les nombres réels
%\newcommand{\R}{\mathrm{R}} 		% pour les Rf_*, etc.
\renewcommand{\L}{\mathrm{L}}		% pour les Lf^* etc.
\newcommand{\RG}{\mathrm{R\Gamma}} 	% pour le RGamma
\newcommand{\HH}{\mathrm{H}} 		% pour les H^i
\newcommand{\SheafRG}{\mathrm{R\mathbf{\Gamma}}} % RGamma "souligné"


\renewcommand{\det}{\mathrm{d\acute{e}t}} % déterminant
\newcommand{\tr}{\mathrm{Tr}}		% trace

% catégories dérivées
\newcommand{\dbc}{\mathsf{D}_c^b} 	% catégorie dérivée bornée
\newcommand{\db}{{\mathsf{D}^b}}	% bornée
\newcommand{\dplus}{{\mathsf{D}^{+}}}	% Dplus
\newcommand{\dbcoh}{\mathsf{D}_{\mathsf{coh}}^b} % bornée à cohomologie cohérente 
\newcommand{\dm}{{\mathsf{D}^{-}}}	% Dmoins
\newcommand{\dmc}{{\mathsf{D}_c^{-}}}
\newcommand{\dtotale}{\mathsf{D}}
\newcommand{\dbctf}{\mathsf{D}_{ctf}^b}
\newcommand{\dbcparf}{\mathsf{D}_{c-parf}^b}
\newcommand{\dbtf}{\mathsf{D}_{tf}^b}


\renewcommand{\ker}{\mathrm{Ker}}
\newcommand{\coker}{\mathrm{Coker}}
\newcommand{\rang}{{\mathrm{rang}}}
\newcommand{\Frac}{{\mathrm{Frac}}}


% l-adique
\newcommand{\QL}{{\QQ_{\ell}}}
\newcommand{\QLB}{{{\sur{\QQ_{\ell}}}}}
\newcommand{\ZL}{{\ZZ_{\ell}}}


% caractères spéciaux
\newcommand{\MM}{\mathfrak{m}}
\newcommand{\vide}{\varnothing}

% flèches diverses
\def\commutatif{\ar@{}[rd]|{\circlearrowleft}}
\def\cartesien{\ar@{}[rd]|{\square}}



\newcommand{\dessusdessous}{\stackrel}
%p. ex. : \dessusdessous{nom}{flèche} écrit « nom » au-dessus de « flèche ».



% catégorique
\newcommand{\colim}{{\mathrm{colim}}} % pour les colimites = limites inductives 
\renewcommand{\lim}{{\mathrm{lim}}} % pour les limites = limites projectives

% bibliographie
%%%%%%%%%%%

\def\sga#1#2#3{[{\bf $\mathbf{SGA\,{#1}}$}~{\sc #2}~#3]} 	% \sga{4}{xv}{prop. 4} cite [SGA 4 XV prop. 4]
\def\sgaquatreetdemi#1#2{[{\bf $\mathbf{SGA\,{4\frac12}}$}~{[#1]}~#2]} %\sgaquatreetdemi{Cycle}{2.2} cite [SGA 4 1/2 [Cycle] 2.2]
\def\ega#1#2{[{\bf \'EGA}~{\sc #1}~#2]} 				% \ega{ii}{8.3} cite [ÉGA II 8.3]
\def\egalong#1#2#3{[{\bf \'EGA}~$\textsc{#1}_{\textrm{#2}}$~#3]} 	% \egalong{iv}{3}{21.4.5} cite [ÉGA IV_3 21.4.5]
\def\egazéro#1#2{[{\bf \'EGA}~$0_{\textsc{#1}}$~#2]}		% \egazéro{iv}{21.5} cite [ÉGA 0_IV 21.5]
\def\ac#1#2#3#4{[{\bf Bourbaki}, A.C.,~{\sc #1}, §#2, N°#3#4]}	% [Bourbaki, A.C., IX, §2, N°4, prop. 7]
\def\accourt#1#2{[{\bf Bourbaki}, A.C.,~{\sc #1}, §#2]}  	% [Bourbaki, A.C., IX, §2]
\def\a#1#2#3#4{[{\bf Bourbaki}, A.,~{\sc #1}, §#2, N°#3\,#4]}	% [Bourbaki, A., IX, §3, N°4, prop. 7]
\def\bbk#1#2#3#4#5{[{\bf Bourbaki}, #1,~{\sc #2}, §#3, N°#4\,#5]} % [Bourbaki, ENS., IX, §3, N°4, prop. 7]

% commandes diverses
\def\mc{\mathscr}	% jolis L ou F calligraphiés
\def\got{\mathfrak}	% pour caractères gothiques : par exemple \got{m}
\def\droit{\mathsf}	% sans sérif (droit)
\def\trdist#1#2#3{ \xymatrix{#1 \ar[rr] & & #2 \ar[dl] \\ & #3 \ar[ul]^{+1} & }} % fait un triangle distingué
\def\chap#1{\widehat{#1}} % met un (grand) chapeau Â
\def\sur{\overline}	% surligne
\def\sous{\underline}	% souligne

